A Miniature Vision-Based Localization System for Indoor Blimps

With increasing attention paid to blimp research, I hope to build an indoor blimp to interact with humans. To begin with, I propose developing a visual localization system to enable blimps to localize themselves in an indoor environment autonomously. This system initially reconstructs an indoor environment by employing Structure from Motion with Superpoint visual features. Next, with the previously built sparse point cloud map, the system generates camera poses by continuously employing pose estimation on matched visual features observed from the map. In this project, the blimp only serves as a reference mobile platform that constrains the weight of the perception system. The perception system contains one monocular camera and a WiFi adaptor to capture and transmit visual data to a ground PC station where the algorithms will be executed. The success of this project will transform remote-controlled indoor blimps into autonomous indoor blimps, which can be utilized for applications such as surveillance, advertisement, and indoor mapping.

==> chapters/theory.tex <==
\chapter{Theory}
In this chapter, the underlying theory for vision-based localization will be presented to provide the reader with the necessary information to understand the topic of vision-based localization.

\section{Camera Model}

\begin{figure}[H]
    \centering
	\includegraphics[width=0.7\textwidth]{figures/theory/figure1.png}
	\caption[Camera Matrix]{Visualization of applying the camera extrinsics will transform a 3D point from global coordinates into the camera coordinate system. Image adopt from \cite{garsten20206dof}}
	\label{fig:camera matrix}
\end{figure}

\begin{figure}[H]
    \centering
	\includegraphics[width=0.7\textwidth]{figures/theory/figure2.png}
	\caption[Calibration Matrix]{Applying the calibration matrix K to a point in camera coordinates will reproject it into the image as a pixel coordinate. Image adopt from \cite{garsten20206dof}}
	\label{fig:calibration matrix}
\end{figure}

The camera model describes the process of projecting a point in the 3D world to a 2D image plane. There are many types of camera models. Different camera models are used to describe different kinds of camera lenses. The simplest camera model is the pinhole camera model. The pinhole camera model is a very common and efficient model that describes image rays pass through a pinhole from the front of the pinhole and generates an image by intersecting the image plane at the back of the pinhole. The pinhole is the camera center where all image rays intersect. The transformation from world coordinates into a pinhole camera can be expressed with the projection matrix.
\begin{equation}
P = K \begin{bmatrix}R & t\end{bmatrix}
\label{eq:1}
\end{equation}
where R is a 3x3 rotation matrix, t is a 3x1 translation vector, and K is a 3x3 calibration matrix. $R$ and $t$ are called the Camera Extrinsics, which provides the camera orientation and position information. $K$ is the Camera Intrinsics, which describes the property of the camera. Unlike the Camera Extrinsics, the Camera Intrinsics do not change when the camera is moving. As seen in \ref{fig:camera matrix}, the rotation $R$ and translation $t$ transform a point from a world coordinate system into a camera coordinate system. As seen in \ref{fig:calibration matrix}, from a camera coordinate system, points can then be reprojected into the pixel coordinate system by applying the camera calibration matrix $K$ because the calibration matrix transformed distances into pixel values. The calibration matrix for a pinhole camera looks like
\begin{equation}
K = \begin{bmatrix} f_x & s & c_x \\ 0 & f_y & c_y \\ 0 & 0 & 1\end{bmatrix}
\label{eq:2}
\end{equation}
where the parameters are; $f_x$ and $f_y$ are the focal lengths along the x and y coordinate axes of the pixel coordinate system. Skew $s$, which describes the tilt of the pixels in the image. Finally, $c_x$ and $c_y$ maps the origin from where the z-axis intersects the image plane to the upper left pixel.

An image pixel coordinate $\begin{bmatrix} u & v \end{bmatrix}^T$ can be calculated by projecting the global point $\begin{bmatrix}X & Y & Z\end{bmatrix}^T$ into the image with the projection matrix:
\begin{equation}
\lambda \underbrace{\begin{bmatrix} u \\ v \\ 1\end{bmatrix}}_{\bar{x}} = P \underbrace{\begin{bmatrix} X \\ Y \\ Z \\ 1\end{bmatrix}}_{\bar{X}}
\label{eq:3}
\end{equation}
where $\lambda$ is a scaling parameter. This compact way of applying $R$, $t$ and $K$ requires the use of homogeneous coordinates. Homogeneous coordinates lift an N-dimensional point to an N+1 dimensional line. With the homogeneous coordinates, translations and projections to can be expressed as matrix multiplications. The N-dimensional point can be retrieved after a transformation by dividing by the last entry and then dropping the last entry.

However, reversing the projection, which is to transform a point from an image into the world coordinate will cause a problem. To project a point, we apply $P$ and divide it with the last entry. But when transforming a point from the image into the world, the last entry is not known. It is not possible to calculate the last entry with a single image. Hence, more than one image is required to recover the 3D point.

\section{RANSAC}
\gls{ransac} is a method for picking random data samples to ensures an outlier free subset of data to a certain degree. In many optimization tasks, the data is not perfect. It contains noisy measurements and outliers. Optimizing for all data can then be challenging. Outliers can be far from a correct measurement, contributing to the cost function's large errors, drowning the effect of errors from accurate measurements. The \gls{ransac} method is widely used to try and find a subset of data that only contains inliers.
\begin{equation}
N = \frac{log(1-p)}{log(1-(1-e)^s)}
\label{eq:6}
\end{equation}

\gls{ransac} is solving a problem of using large input data and a solver to compute a solution. The merit of \gls{ransac} is that it can pick a subset of data within the large dataset, which is nearly outlier free, resulting the correct solution's computation. \gls{ransac} randomly picks a subset of $s$ data points $N$ number of times. $N$ is calculated by \ref{eq:6}, where  $e$ is the ratio between outliers and all matched points, and $p$ represents the desired probability of finding the best solution or model. The outlier ratio $e$ is hard to determine and scarcely available. It can, therefore, be necessary to update the distribution based on inlier results calculated during runtime. 

For each iteration, it calculates a solution based on the $s$ data points. Then it calculates an error value for each point within the $s$ points by fitting the point into the solution. For points with an error smaller than a pre-determined threshold are considered as inliers. This procedure is done for all points and will give the number of inliers for a given solution. The number of inliers is used to calculate a new outlier ratio and is then inserted back in \ref{eq:6} to calculate the number of iterations needed. Now, each subset $s$ will be associated with a number of inliers and a solution. After all the iterations, the subset $s$ with the maximum inliers is considered as the best subset and the solution associated with the subset is considered the final solution.

\section{A Structure From motion Pipeline}
The goal of \gls{sfm} is to recover the 3D stationary scene and camera poses with a set of 2D images. An SfM pipeline contains five main steps:

1. Image undistortion.

2. Extract key points and compute descriptors. 

3. Feature Matching.

4. Compute camera poses and reconstruct 3D points.

5. Register 3D model to the real scale and position of the stationary scene.

Image undistortion is to correct the non-linear projection of the surface points of objects onto the image plane due to lens distortion. There are two common types of distortion, tangential distortion and radial distortion. These two types of distortion can be correct with a five parameters undistortion model.

a. Assuming a point $P=\begin{bmatrix} X & Y & Z \end{bmatrix} ^ T$ in the camera frame, its coordinate in the normalized camera frame is:
\begin{equation}
\begin{bmatrix} x \\ y  \end{bmatrix}=\begin{bmatrix} X/Z \\ Y/Z \end{bmatrix}
\end{equation}

b. Correct tangential distortion and radial distortion in the normalized camera frame:
\begin{equation}
\begin{split}
    x_{distort} = x(1+k_1r^2+k_2r^4+k_3r^6)+2p_1xy+p_2(r^2+2x^2)\\
    y_{distort} = y(1+k_1r^2+k_2r^4+k_3r^6)+p_1(r^2+2y^2)+2p_2xy
\end{split}
\label{eq:3.3.2}
\end{equation}


c. Finally, project the new point into the pixel coordinate will get the correct position of the point in the image.

% \begin{figure}[H]
%     \centering
% 	\includegraphics[width=0.7\textwidth]{figures/theory/image gradient.png}
% 	\caption[Image gradient]{Image gradient computation into keypoint descriptors. Image adopt from \cite{garsten20206dof}}
% 	\label{fig:image gradient}
% \end{figure}

The process of extracting key points and computing descriptors is called feature extraction. This process is to find representative points that can describe an image in a compression way. These points can still be found in an image when the camera field of view sightly changes. Descriptors are information encoded into features to discriminate features from each other. The most common feature descriptor is SIFT. Sift key point is obtained by sliding a Difference of Gaussian filter over the image and detecting local extrema for the filter. The descriptor of Sift is a 128 length vector describing the gradients around the key point.

Feature Matching is to compare feature descriptors across the images to identify similar features. Comparing descriptors is done by computing the Euclidean distance between them. Because descriptors are usually high dimensional vectors, comparing descriptors from two sets of features is expensive. Approximate search is used instead of exhaustively looking for the best match to decrease the matching time. This approximate search is done by arranging all data into a k-d tree (k-dimensional tree). Similar data that has the best matches can be found by following the path down the top of the tree. To further ensure that good matches are found it is common to use Lowe's ratio test to discard matches that are probably to be false. The ratio test takes the ratio of the distance between the first and second nearest neighbors of the descriptor to be matched and evaluates if the ratio is less than a pre-defined threshold. The first nearest neighbor is the most similar descriptor to the matched descriptor, while the second nearest neighbor is the second most similar descriptor. This is expressed as
\begin{equation}
    \frac{|d_i - d_{N1}|^2}{|d_i - d_{N2}|^2}\leq tol
\end{equation}
where $d_i$ is the descriptor to be matched, $d_{N1}$ and $d_{N2}$ are the first and second nearest neighbor matches and $tol$ is the predefined tolerance. A match passes the ratio test if the ratio is below the threshold. Employing the ratio test ensures that matched descriptors are more similar to each other than to other descriptors. This filters out matches that are unlikely to be correct. However, in most of the case, a ratio test cannot eliminate false positives. Next, using the RANSCAC algorithm to find the geometry constraint, such as homography matrix, fundamental matrix or essential matrix if the camera calibration matrix is known, can filter bad matches further.

There are two ways to reconstruct the 3D points and compute the camera poses, incrementally or globally. Global SfM estimates all camera positions and 3D points at the same time. In contrast, incremental SfM finds a good starting image pair to create an initial model. Given this initial model, one by one images are added to the model. Each new image has to see n 3D points already in the model for a camera pose to be computed. The number of points depend on how much information is available about the camera and also determines which PnP solver to be used. New point correspondences can then be triangulated and added to the point cloud. As more images are added, small errors will accumulate, distorting the model. It is common to perform optimization on both 3D point and camera poses with set intervals.   

Optimization or more specifically, bundle adjustment is performed to minimize growing errors by shifting the position of 3D points and, depending on how much information about the camera is known, tuning the projection matrix. Localization error is usually quantified as the reprojection error of 3D points. It is computed by taking the square of all 2D image points subtracted by their respectively reprojected 3D point correspondence as

\begin{equation}
    e = \sum_{i=1}^{n}\sum_{j=1}^{m}\norm{(x_{ij} - \frac{p^1_i\mathbf{X}_j}{p^3_i\mathbf{X}_j}),(y_{ij} -\frac{p^2_i\mathbf{X}_j}{p^3_i\mathbf{X}_j})}^2
\end{equation}


The final reconstructed 3D model, however, is under a scale ambiguity. Normally, a similarity transform will be applied to recale the model and transform it to a new position and orientation. 

\begin{equation}
    T_s = \begin{bmatrix} sR & t \\ 0 & 1\end{bmatrix}
\end{equation}
where $s$ is the scaling factor, $R$ is a 3x3 rotation matrix and $t$ is a 3x1 translation vector. 


% \section{A Structure From motion Pipeline}
% The goal of \gls{sfm} is to recover the 3D stationary scene and camera poses with a set of 2D images. An SfM pipeline contains four main steps:

% 1. Image rectification. This is to correct the distortion caused by camera lens.

% 2. Extract image features and compute descriptors. To compare images against each other, it is possible to use individual pixel values or a blurred version to see if general patterns match. However, this yields poor results, and unique features are instead computed.

% 2. Match descriptors. With sufficiently unique features, they can now be matched to determine if the same feature is present in multiple images.

% 3. Estimate camera positions and create point cloud model. Matched features can now be triangulated into 3D points. This can be done either by Incremental \gls{sfm} or Global \gls{sfm}.

% \begin{figure}[H]
%     \centering
% 	\includegraphics[width=0.7\textwidth]{figures/theory/image gradient.png}
% 	\caption[Image gradient]{Image gradient computation into keypoint descriptors.}
% 	\label{fig:image gradient}
% \end{figure}

% In image processing, feature extraction extracts key points from an image and compute descriptors to describe each key point. The most common feature descriptor is SIFT. Sift feature is obtained by sliding a Difference of Gaussian filter over the image and detecting local extrema for the filter. Different descriptors have different ways of computation, but a common descriptor such as SIFT uses gradient vectors to describe features. As seen in \ref{fig:image gradient}, gradients are created by analyzing a small portion of the image and creating gradients to nearby pixels based on changes in light intensity. All gradients are then placed into the bins of multiple histograms, which are concatenated to form a descriptor. When creating a descriptor, the goal is to make it as robust and unique as possible. A robust descriptor will not change in different lighting and weather conditions. This is an important characteristic for matching features in images taken over long periods of time. Uniqueness in the other hand is important as to not match descriptors which do not represent the same point, so called false positives.

% Matching descriptors to one another is a simple task in theory. As with simple 3D points, comparing descriptors is done by computing the Euclidean distance between them. What may not be obvious is that with high dimensional data such as descriptors, this distance will be large even to close matches. Close matches will have many dimensions that match well but some will not and this is enough for distances to grow large. High dimensional data is also usually gathered in large quantities because of the larger space they reside in. This makes matching all descriptors a non trivial task that can take lots of time. To decrease the time spent matching, approximate search is used instead of exhaustively looking for the best match. Approximate search can be done by arranging all data into a k-d tree (k-dimensional tree). Arranging the data in a tree structure makes it easier to only search data that is similar. Starting from the top of the tree, similar data can be found by following the path down the tree which has the best matches. To further ensure that good matches are found it is common to use Lowe's ratio test to discard matches that are probable to be false. The ratio test takes the ratio of the distance between the first and second nearest neighbors of the descriptor to be matched and evaluates if the ratio is less than a pre-defined threshold. The first nearest neighbor is the most similar descriptor to the matched descriptor while the second nearest neighbor is the second most similar descriptor. This is expressed as
% \begin{equation}
%     \frac{|d_i - d_{N1}|^2}{|d_i - d_{N2}|^2}\leq tol
% \end{equation}
% where $d_i$ is the descriptor to be matched, $d_{N1}$ and $d_{N2}$ are the first and second nearest neighbor matches and $tol$ is the predefined tolerance. A match passes the ratio test if the ratio is below the threshold. Employing the ratio test ensures that matched descriptors are more similar to each other than to other descriptors. This filters out matches that are unlikely to be correct. However, in most of the case a ratio test cannot completely eliminate false positives. Next using RANSCAC algorithm to find the geometry constraint, such as homography matrix, fundamental matrix or essential matrix if the camera calibration matrix is known, can further filter bad matches.

% Creating a point cloud model can be done in two ways, incrementally or globally. Incremental SfM adds one image at a time to the reconstruction, incrementally expanding the model. Global SfM estimates all camera positions at the same time by first constructing a graph connecting cameras viewing the same scene. Only incremental SfM will be explained here.

% Incremental SfM first finds a good starting image pair from which an initial model can be created. Given this initial model, one by one images are added to the model. Each new image has to see n 3D points already in the model for a camera pose to be computed. The number of points depend on how much information is available about the camera and also determines which PnP solver to be used. New point correspondences can then be triangulated and added to the point cloud. As more images are added, small errors will accumulate distorting the model. It is common to perform optimization on both 3D point and camera poses with set intervals.

% Optimization or more specifically bundle adjustment is performed to minimize growing errors by shifting the position of 3D points and, depending on how much information about the camera is known, tuning the projection matrix. Localization error is usually quantified as the reprojection error of 3D points. It is computed by taking the square of all 2D image points subtracted by their respectively reprojected 3D point correspondence as

% \begin{equation}
%     e = \sum_{i=1}^{n}\sum_{j=1}^{m}\norm{(x_{ij} - \frac{p^1_i\mathbf{X}_j}{p^3_i\mathbf{X}_j}),(y_{ij} -\frac{p^2_i\mathbf{X}_j}{p^3_i\mathbf{X}_j})}^2
% \end{equation}

\section{Perspective-n-Point}

 Perspective-n-Point (PnP) is the problem of estimating the pose of a calibrated camera given a set of n 3D points in the world and their corresponding 2D projections in the image. A camera matrix has the dimensions of 3x4, containing twelve variables. We only have to solve eleven variables as it is determined up to an arbitrary scale. To solve eleven variables, eleven equations are required. The camera gives three equations for every point but $\lambda$ also has to be solved for each new point. The number of points required then becomes
\begin{equation}
    3n > 11+n \Rightarrow n \geq 5.5
    \label{eq:3.4.1}
\end{equation}

A simple approach to solve systems of linear equations is called direct linear transform (DLT). This approach expresses all equations in terms of a matrix multiplication and finds an approximate nullspace for the matrix. The DLT algorithm
explained below is a slightly modified version of the one in \cite{hartley2003multiple}. First, lets express P as
\begin{equation}
    P = \begin{bmatrix} p_1 \\ p_2 \\ p_3\end{bmatrix}
    \label{eq:3.4.2}
\end{equation}

where $p_i$, $i$ = 1, 2, 3, are 1x4 row vectors from $P$. Insert this representation of $P$ into \ref{eq:3} and it can be written as
\begin{equation}
\begin{split}
    p_1 X - \lambda x = 0\\
    p_2 X - \lambda y = 0\\
    p_3 X - \lambda = 0\\
\end{split}
\label{eq:3.4.3}
\end{equation}

which in matrix form looks like

\begin{equation}
    \begin{bmatrix} 
        X^T & 0 & 0 & -x \\ 
        0 & X^T & 0 & -y \\
        0 & 0 & X^T & -1 \\
    \end{bmatrix} \begin{bmatrix} p^T_1 \\ p^T_2 \\ p^T_3 \\ \lambda \end{bmatrix}= 
    \begin{bmatrix} 0 \\ 0 \\ 0 \end{bmatrix}
     \label{eq:3.4.4}
\end{equation}

This is the matrix for only a single point. To find $P$ at least 6 points are required
according to \ref{eq:3.4.1}. If we include more points in \ref{eq:3.4.4} the matrix will be on the form

\begin{equation}
    \underbrace{\begin{bmatrix} 
    X^T_1 & 0 & 0 & -x_1 & 0 & 0 & \cdots \\ 
    0 & X^T_1 & 0 & -y_1 & 0 & 0 & \cdots\\ 
    0 & 0 & X^T_1 & -1 & 0 & 0 & \cdots\\ 
    X^T_2 & 0 & 0 & 0 & -x_2 & 0 & \cdots\\ 
    0 & X^T_2 & 0 & 0 & -y_2 & 0 & \cdots\\ 
    0 & 0 & X^T_2 & 0 & -1 & 0 & \cdots\\ 
    X^T_3 & 0 & 0 & 0 & 0 & -x_3 & \cdots\\ 
    0 & X^T_3 & 0 & 0 & 0 & -y_3 & \cdots\\ 
    0 & 0 & X^T_3 & 0 & 0 & -1 & \cdots\\ 
    \vdots & \vdots & \vdots & \vdots & \vdots & \vdots &\ddots
    \end{bmatrix}}_{M}\underbrace{\begin{bmatrix}p^T_1 \\ p^T_2 \\ p^T_3 \\ \lambda_1\\ \lambda_2\\ \lambda_3 \\ \vdots\end{bmatrix}}_{v} = \begin{bmatrix}0\\0\\0\\0\\0\\0\\ \vdots\end{bmatrix}
\end{equation}

This equation can be solved by finding a non-zero vector in the nullspace of M. Since the scale of the solution is arbitrary the constraint $\norm{v}^2 = 1$ can be applied. This system will most likely not have an exact solution and a least squares solution is found by minimizing:

\begin{equation}
    \underset{\norm{v}^2=1}{min} \norm{Mv}^2
\end{equation}



\section{Factor Graph}
Factor Graph were define by as Factor graphs are graphical models (\cite{koller2009probabilistic}) that are well suited to modeling complex estimation problems, such as Simultaneous Localization and Mapping or \gls{sfm}. Different from a more common graphic model Bayes networks, which are directed acyclic graphs, a factor graph, however, is a bipartite graph consisting of factors connected to variables. The variables represent the unknown random variables in the estimation problem, whereas the factors represent probabilistic information on those variables, derived from measurements or prior knowledge. (\cite{Dellaert2012factor})
